Asymmetric Feature Fusion for Image Retrieval

In asymmetric retrieval systems, models with different capacities are deployed on platforms with different computational and storage resources. Despite the great progress, existing approaches still suffer from a dilemma between retrieval efficiency and asymmetric accuracy due to the limited capacity of the lightweight query model. In this work, we propose an Asymmetric Feature Fusion (AFF) paradigm, which advances existing asymmetric retrieval systems by considering the complementarity among different features just at the gallery side. Specifically, it first embeds each gallery image into various features, e.g., local features and global features. Then, a dynamic mixer is introduced to aggregate these features into compact embedding for efficient search. On the query side, only a single lightweight model is deployed for feature extraction. The query model and dynamic mixer are jointly trained by sharing a momentum-updated classifier. Notably, the proposed paradigm boosts the accuracy of asymmetric retrieval without introducing any extra overhead to the query side. Exhaustive experiments on various landmark retrieval datasets demonstrate the superiority of our paradigm.

==> plots/Mixer_LAFF.tex <==
\begin{tikzpicture}[font={\footnotesize},]
	\node[] at (0, 125pt) (i1){$\bm{f}^1$};
	\node[] at (30pt, 125pt) (i2){$\cdots$};
	\node[] at (60pt, 125pt) (i3){$\bm{f}^K$};
	
	\node[cat] at (0, 100pt) (t1){tanh};
	\node[](t2) at (30pt, 100pt) {$\cdots$};
	\node[cat] at (60pt, 100pt) (t3){tanh};
	
	\node[op] at (30pt, 87.5pt) (cat){$+$};  
	
	\node[fill=blue!10,draw,minimum width=50pt,inner sep=2pt] at (30pt, 65pt) (d1){Linear}; 
	\node[fill=red!15,draw,minimum width=50pt,inner sep=2pt] at (30pt, 42.5pt) (soft){Softmax};
	
	\node[op] at (30pt, 20pt) (mul){$\times$};
	\node[] at (30pt, 0pt) (out){$\bm{f}^{\text{fusion}}$};
	
	\coordinate(f) at($(cat.south)!.5!(d1.north)$); % split
	\node(residual)[left=5pt of d1.west]{};
	\coordinate(re) at(residual.center);
	
	\coordinate(f2) at($(soft.south)+ (0, -0.25)$); % split
	
	\draw[->] (i1) edge node[dim,midway,right]{$1 \times d^*$} (t1);
	\draw[->] (i3) edge node[dim,midway,right]{$1 \times d^*$} (t3);
	
	\draw[->] (d1) edge node[dim,midway,right]{$K \times 1$} (soft);
	\draw[->] (soft) edge node[dim,midway,right]{$K \times 1$} (mul);
	\draw[->] (mul) edge node[dim,midway,right]{$1 \times d^*$} (out);
	
	\draw[->] (t1) |- (cat);
	\draw[->] (t3) |- (cat);
	\draw[->] (cat) -- node[dim,midway,right]{$K \times d^*$} (d1);
	
	
	\draw (f) -| (re) (re) |- (mul);
\end{tikzpicture}

==> plots/Mixer_Orth.tex <==
\begin{tikzpicture}[font={\footnotesize},]
	
	\node[] at (0, 125pt) (f1){$\bm{f}^1,\cdots,\bm{f}^K$};  
	\node[gap] at (54pt, 125pt) (f2){GAP};  
	\node[] at (90pt, 125pt) (f3){$\bm{f}^{g}$};
	\draw[->] (f1) edge (f2);  
	\draw[->] (f2) edge (f3);
	
	\node[draw,fill=orange!50,minimum width=110pt,minimum height=15pt] at(45pt,93pt) (proj){Project: $\bm{p}_i = \frac{\bm{f}_i\bm{f}_g^T}{||\bm{f}^g||_2^2}\bm{f}^g$};
	
	\coordinate(a1) at($(f1.south) + (0, -12pt)$); % split
	\draw[->] (f1) edge node[dim,midway,right]{$K \times d^*$} (a1);
	
	\coordinate(a2) at($(f3.south) + (0, -13pt)$); % split
	\draw[->] (f3) edge (a2);
	
	\coordinate(a3) at($(f1.south) + (0, -4pt)$); % split
	\coordinate(a4) at($(proj.west) + (-10pt,0pt)$); % split
	\draw (a3) -| (a4);
	
	\node[op] at(45pt, 65pt) (cat){$+$};
	
	\node[op] at(0pt,65pt) (diff){$-$};
	\draw[->] (a4) |- (diff);
	
	\node[] at($(f1.south) + (0, -33pt)$) (a5){}; % split
	\draw[->] (a5) edge (diff);
	
	\coordinate(a6) at($(f3.south) + (0, -3pt)$); % split
	\coordinate(a7) at($(proj.east) + (10pt,0pt)$); % split
	\draw (a6) -| (a7);
	\draw[->] (a7) |-  (cat);
	\draw[->] (diff) edge node[dim,midway,above]{$K \times d^*$} (cat);
	\node[dim] at (80pt,71.8pt) {$1 \times d^*$};
	
	\node[fill=brown!25,draw,minimum width=50pt,inner sep=2pt] at(45pt,44pt) (avg){GAP};
	\node[fill=blue!10,draw,minimum width=50pt,inner sep=2pt] at(45pt,23pt) (linear){Linear};
	
	\draw[->] (cat) edge node[dim,midway,right]{$K \times 2d^{*}$} (avg);
	\draw[->] (avg) edge node[dim,midway,right]{$1 \times 2d^{*}$} (linear);
	
	\node[] at (45pt,0pt) (out){$\bm{f}_{\text{fusion}}$};
	\draw[->] (linear) edge node[dim,midway,right]{$1 \times d^{*}$} (out);
	
\end{tikzpicture}
